Training Data for Large Language Model

In 2022, with the release of ChatGPT, large-scale language models gained widespread attention. ChatGPT not only surpassed previous models in terms of parameters and the scale of its pretraining corpus but also achieved revolutionary performance improvements through fine-tuning on a vast amount of high-quality, human-annotated data. This progress has led enterprises and research institutions to recognize that building smarter and more powerful models relies on rich and high-quality datasets. Consequently, the construction and optimization of datasets have become a critical focus in the field of artificial intelligence. This paper summarizes the current state of pretraining and fine-tuning data for training large-scale language models, covering aspects such as data scale, collection methods, data types and characteristics, processing workflows, and provides an overview of available open-source datasets.

==> ccl_jym.tex <==
% File ccl2023-zh.sty
%
% This is the LaTeX style file for CCL 2023.
% Contact: zhangyue@westlake.edu.cn
%%
%% Based on the original version of COLING-2018 file (coling2018.sty), with changes made by Yue Zhang.
%%

% Papers are to be prepared using the ``acl'' bibliography style,
% as follows:
%       \documentclass[11pt]{article}
%       \usepackage{acl2000}
%       \title{Title}
%       \author{Author 1 \and Author 2 \\ Address line \\ Address line \And
%               Author 3 \\ Address line \\ Address line}
%       \begin{document}
%       ...
%       \bibliography{bibliography-file}
%       \bibliographystyle{acl}
%       \end{document}

% Author information can be set in various styles:
% For several authors from the same institution:
% \author{Author 1 \and ... \and Author n \\
%         Address line \\ ... \\ Address line}
% if the names do not fit well on one line use
%         Author 1 \\ {\bf Author 2} \\ ... \\ {\bf Author n} \\
% For authors from different institutions:
% \author{Author 1 \\ Address line \\  ... \\ Address line
%         \And  ... \And
%         Author n \\ Address line \\ ... \\ Address line}
% To start a seperate ``row'' of authors use \AND, as in
% \author{Author 1 \\ Address line \\  ... \\ Address line
%         \AND
%         Author 2 \\ Address line \\ ... \\ Address line \And
%         Author 3 \\ Address line \\ ... \\ Address line}

% If the title and author information does not fit in the area allocated,
% place \setlength\titlebox{<new height>} right after
% \usepackage{ccl2020-zh}
% where <new height> can be something larger than 5cm

\typeout{Conference Style for CCL 2023 -- prepared 19th Dec. 2019}

% NOTE:  Some laser printers have a serious problem printing TeX output.
% These printing devices, commonly known as ``write-white'' laser
% printers, tend to make characters too light.  To get around this
% problem, a darker set of fonts must be created for these devices.
%


% include hyperref, unless user specifies nohyperref option like this:
% \usepackage[nohyperref]{ccl2020-en}
\newif\ifccl@hyperref
\DeclareOption{hyperref}{\ccl@hyperreftrue}
\DeclareOption{nohyperref}{\ccl@hyperreffalse}
\ProcessOptions\relax
\ifccl@hyperref
  \usepackage{hyperref}
  \usepackage{xcolor}		% make links dark blue
  \definecolor{darkblue}{rgb}{0, 0, 0.5}
  \hypersetup{colorlinks=true,citecolor=darkblue, linkcolor=darkblue, urlcolor=darkblue}
\else
  % This definition is used if the hyperref package is not loaded.
  % It provides a backup, no-op definiton of \href.
  \def\href#1#2{{#2}}
  % We still need to load xcolor in this case because the lighter line numbers require it. (SC/KG/WL) 
  \usepackage{xcolor}

  % Code taken from
  % https://tex.stackexchange.com/questions/124410/hyperref-modifies-bibliography-style-of-acl-style-files
  % which fixes incorrect bibliography styles when using the hyperref package
  \newcommand{\@BIBLABEL}{\@emptybiblabel}
\fi
\newcommand{\@emptybiblabel}[1]{}

% footnote without an anchor
\newcommand\cclfootnote[1]{%
  \begin{NoHyper}
  \renewcommand\thefootnote{}\blfootnote{#1}%
  \addtocounter{footnote}{-1}%
  \end{NoHyper}
}


% A4 modified by Eneko; again modified by Alexander for 5cm titlebox
\setlength{\paperwidth}{21cm}   % A4
\setlength{\paperheight}{29.7cm}% A4
\setlength\topmargin{-1.2cm}    
\setlength\oddsidemargin{0cm}   
\setlength\textheight{24.7cm} 
\setlength\textwidth{16.0cm}
\setlength\columnsep{0.6cm}  
\newlength\titlebox 
\setlength\titlebox{5cm}
\setlength\headheight{15pt}   
\setlength\headsep{2em}
\thispagestyle{empty}        
\pagestyle{empty}

\flushbottom \sloppy

% We're never going to need a table of contents, so just flush it to
% save space --- suggested by drstrip@sandia-2
\def\addcontentsline#1#2#3{}

% Footnote without marker for copyright/licence statement
% Code taken from
% http://tex.stackexchange.com/questions/30720/footnote-without-a-marker
% which claims to have taken it, in turn, from
% http://help-csli.stanford.edu/tex/latex-footnotes.shtml#unnumber
% Note the comment that there may be numbering problems if
% you are using the hyperref package. 
\def\blfootnote{\xdef\@thefnmark{}\@footnotetext}

% Title stuff, taken from deproc.
\def\maketitle{\par
 \begingroup
   \def\thefootnote{\fnsymbol{footnote}}
   \def\@makefnmark{\hbox to 0pt{$^{\@thefnmark}$\hss}}
   \@maketitle \@thanks
 \endgroup
 \setcounter{footnote}{0}
 \let\maketitle\relax \let\@maketitle\relax
 \gdef\@thanks{}\gdef\@author{}\gdef\@title{}\let\thanks\relax}
\def\@maketitle{\vbox to \titlebox{\hsize\textwidth
 \linewidth\hsize \vskip 0.125in minus 0.125in \centering
 {\Large\bf \@title \par} \vskip 0.2in plus 1fil minus 0.1in
 {\def\and{\unskip\enspace{\rm and}\enspace}%
  \def\And{\end{tabular}\hss \egroup \hskip 1in plus 2fil 
           \hbox to 0pt\bgroup\hss \begin{tabular}[t]{c}\bf}%
  \def\AND{\end{tabular}\hss\egroup \hfil\hfil\egroup
          \vskip 0.25in plus 1fil minus 0.125in
           \hbox to \linewidth\bgroup\large \hfil\hfil
             \hbox to 0pt\bgroup\hss \begin{tabular}[t]{c}\bf}
  \hbox to \linewidth\bgroup\large \hfil\hfil
    \hbox to 0pt\bgroup\hss \begin{tabular}[t]{c}\bf\@author 
                            \end{tabular}\hss\egroup
    \hfil\hfil\egroup}
  \vskip 0.3in plus 2fil minus 0.1in
}}

% margins for abstract
\renewenvironment{abstract}%
		 {\centerline{\large\bf 摘要}%
		  \begin{list}{}%
		     {\setlength{\rightmargin}{2em}%
		      \setlength{\leftmargin}{2em}}%
              \item[]\ignorespaces}%
		 {\unskip\end{list}}


% Keywords
\def\keywordname{{\bf 关键词：}}%
\def\keywords#1{\par\addvspace\medskipamount{\rightskip=0pt plus1cm
\def\and{\ifhmode\unskip\nobreak\fi\ ；
}\keywordname\enspace\ignorespaces#1\par}}


% For English title and authors
\newcommand\@englishtitle{}
\newcommand\englishtitle[1]{\renewcommand\@englishtitle{#1} \relax}

\newcommand\@englishauthor{}
\newcommand\englishauthor[1]{\renewcommand\@englishauthor{#1} \relax}

\def\makeenglishtitle{\par \@makeenglishtitle 
 \let\maketitle\relax \let\@makeenglishtitle\relax}
\def\@makeenglishtitle{\vbox to \titlebox{\hsize\textwidth
 \linewidth\hsize \vskip 0.125in minus 0.125in \centering
 {\Large\bf \@englishtitle \par} \vskip 0.2in plus 1fil minus 0.1in
 {\def\and{\unskip\enspace{\rm and}\enspace}%
  \def\And{\end{tabular}\hss \egroup \hskip 1in plus 2fil 
           \hbox to 0pt\bgroup\hss \begin{tabular}[t]{c}\bf}%
  \def\AND{\end{tabular}\hss\egroup \hfil\hfil\egroup
          \vskip 0.25in plus 1fil minus 0.125in
           \hbox to \linewidth\bgroup\large \hfil\hfil
             \hbox to 0pt\bgroup\hss \begin{tabular}[t]{c}\bf}
  \hbox to \linewidth\bgroup\large \hfil\hfil
    \hbox to 0pt\bgroup\hss \begin{tabular}[t]{c}\bf\@englishauthor 
                            \end{tabular}\hss\egroup
    \hfil\hfil\egroup}
  \vskip 0.3in plus 2fil minus 0.1in
}}

% margins for English abstract
\newenvironment{englishabstract}%
		 {\vskip 0.125in minus 0.125in\centerline{\large\bf Abstract}%
		  \begin{list}{}%
		     {\setlength{\rightmargin}{2em}%
		      \setlength{\leftmargin}{2em}}%
              \item[]\ignorespaces}%
		 {\vskip 0.3in minus 0.1in\end{list}}

% English keywords
\def\englishkeywordname{{\bf Keywords: }}%
\def\englishkeywords#1{\par\addvspace\medskipamount{\rightskip=0pt plus1cm
\def\and{\ifhmode\unskip\nobreak\fi\ ,
}{\setlength{\leftmargin}{2em}
  \flushleft{\englishkeywordname\enspace\ignorespaces#1}\par}}}


% bibliography
\def\thebibliography#1{\section*{References}
  \global\def\@listi{\leftmargin\leftmargini
               \labelwidth\leftmargini \advance\labelwidth-\labelsep
               \topsep 1pt plus 2pt minus 1pt
               \parsep 0.25ex plus 1pt \itemsep 0.25ex plus 1pt}
  \list {[\arabic{enumi}]}{\settowidth\labelwidth{[#1]}\leftmargin\labelwidth
    \advance\leftmargin\labelsep\usecounter{enumi}}
    \def\newblock{\hskip .11em plus .33em minus -.07em}
    \sloppy
    \sfcode`\.=1000\relax}

\def\@up#1{\raise.2ex\hbox{#1}}

% most of cite format is from aclsub.sty by SMS

% don't box citations, separate with ; and a space
% also, make the penalty between citations negative: a good place to break
% changed comma back to semicolon pj 2/1/90
% \def\@citex[#1]#2{\if@filesw\immediate\write\@auxout{\string\citation{#2}}\fi
% \def\@citea{}\@cite{\@for\@citeb:=#2\do
%   {\@citea\def\@citea{;\penalty\@citeseppen\ }\@ifundefined
%      {b@\@citeb}{{\bf ?}\@warning
%      {Citation `\@citeb' on page \thepage \space undefined}}%
% {\csname b@\@citeb\endcsname}}}{#1}}

% don't box citations, separate with ; and a space
% Replaced for multiple citations (pj) 
% don't box citations and also add space, semicolon between multiple citations
\def\@citex[#1]#2{\if@filesw\immediate\write\@auxout{\string\citation{#2}}\fi
  \def\@citea{}\@cite{\@for\@citeb:=#2\do
     {\@citea\def\@citea{; }\@ifundefined
       {b@\@citeb}{{\bf ?}\@warning
        {Citation `\@citeb' on page \thepage \space undefined}}%
 {\csname b@\@citeb\endcsname}}}{#1}}

% Allow short (name-less) citations, when used in
% conjunction with a bibliography style that creates labels like
%       \citename{<names>, }<year>
% 
\let\@internalcite\cite
\def\cite{\def\citename##1{##1, }\@internalcite}
\def\shortcite{\def\citename##1{}\@internalcite}
\def\newcite{\def\citename##1{{\frenchspacing##1} (}\@internalciteb}

% Macros for \newcite, which leaves name in running text, and is
% otherwise like \shortcite.
\def\@citexb[#1]#2{\if@filesw\immediate\write\@auxout{\string\citation{#2}}\fi
  \def\@citea{}\@newcite{\@for\@citeb:=#2\do
    {\@citea\def\@citea{;\penalty\@m\ }\@ifundefined
       {b@\@citeb}{{\bf ?}\@warning
       {Citation `\@citeb' on page \thepage \space undefined}}%
{\csname b@\@citeb\endcsname}}}{#1}}
\def\@internalciteb{\@ifnextchar [{\@tempswatrue\@citexb}{\@tempswafalse\@citexb[]}}

\def\@newcite#1#2{{#1\if@tempswa, #2\fi)}}

\def\@biblabel#1{\def\citename##1{##1}[#1]\hfill}

%%% More changes made by SMS (originals in latex.tex)
% Use parentheses instead of square brackets in the text.
\def\@cite#1#2{({#1\if@tempswa , #2\fi})}

% Don't put a label in the bibliography at all.  Just use the unlabeled format
% instead.
\def\thebibliography#1{\vskip\parskip%
\vskip\baselineskip%
\def\baselinestretch{1}%
\ifx\@currsize\normalsize\@normalsize\else\@currsize\fi%
\vskip-\parskip%
\vskip-\baselineskip%
\section*{参考文献\@mkboth
 {References}{References}}\list
 {}{\setlength{\labelwidth}{0pt}\setlength{\leftmargin}{\parindent}
 \setlength{\itemindent}{-\parindent}}
 \def\newblock{\hskip .11em plus .33em minus -.07em}
 \sloppy\clubpenalty4000\widowpenalty4000
 \sfcode`\.=1000\relax}
\let\endthebibliography=\endlist

% Allow for a bibliography of sources of attested examples
\def\thesourcebibliography#1{\vskip\parskip%
\vskip\baselineskip%
\def\baselinestretch{1}%
\ifx\@currsize\normalsize\@normalsize\else\@currsize\fi%
\vskip-\parskip%
\vskip-\baselineskip%
\section*{Sources of Attested Examples\@mkboth
 {Sources of Attested Examples}{Sources of Attested Examples}}\list
 {}{\setlength{\labelwidth}{0pt}\setlength{\leftmargin}{\parindent}
 \setlength{\itemindent}{-\parindent}}
 \def\newblock{\hskip .11em plus .33em minus -.07em}
 \sloppy\clubpenalty4000\widowpenalty4000
 \sfcode`\.=1000\relax}
\let\endthesourcebibliography=\endlist

\def\@lbibitem[#1]#2{\item[]\if@filesw 
      { \def\protect##1{\string ##1\space}\immediate
        \write\@auxout{\string\bibcite{#2}{#1}}\fi\ignorespaces}}

\def\@bibitem#1{\item\if@filesw \immediate\write\@auxout
       {\string\bibcite{#1}{\the\c@enumi}}\fi\ignorespaces}

% sections with less space
\def\section{\@startsection {section}{1}{\z@}{-2.0ex plus
    -0.5ex minus -.2ex}{1.5ex plus 0.3ex minus .2ex}{\large\bf\raggedright}}
\def\subsection{\@startsection{subsection}{2}{\z@}{-1.8ex plus
    -0.5ex minus -.2ex}{0.8ex plus .2ex}{\normalsize\bf\raggedright}}
%% changed by KO to - values to get teh initial parindent right
\def\subsubsection{\@startsection{subsubsection}{3}{\z@}{-1.5ex plus
   -0.5ex minus -.2ex}{0.5ex plus .2ex}{\normalsize\bf\raggedright}}
\def\paragraph{\@startsection{paragraph}{4}{\z@}{1.5ex plus
   0.5ex minus .2ex}{-1em}{\normalsize\bf}}
\def\subparagraph{\@startsection{subparagraph}{5}{\parindent}{1.5ex plus
   0.5ex minus .2ex}{-1em}{\normalsize\bf}}

% Footnotes
\footnotesep 6.65pt %
\skip\footins 9pt plus 4pt minus 2pt
\def\footnoterule{\kern-3pt \hrule width 5pc \kern 2.6pt }
\setcounter{footnote}{0}

% Lists and paragraphs
\parindent 1em
\topsep 4pt plus 1pt minus 2pt
\partopsep 1pt plus 0.5pt minus 0.5pt
\itemsep 2pt plus 1pt minus 0.5pt
\parsep 2pt plus 1pt minus 0.5pt

\leftmargin 2em \leftmargini\leftmargin \leftmarginii 2em
\leftmarginiii 1.5em \leftmarginiv 1.0em \leftmarginv .5em \leftmarginvi .5em
\labelwidth\leftmargini\advance\labelwidth-\labelsep \labelsep 5pt

\def\@listi{\leftmargin\leftmargini}
\def\@listii{\leftmargin\leftmarginii
   \labelwidth\leftmarginii\advance\labelwidth-\labelsep
   \topsep 2pt plus 1pt minus 0.5pt
   \parsep 1pt plus 0.5pt minus 0.5pt
   \itemsep \parsep}
\def\@listiii{\leftmargin\leftmarginiii
    \labelwidth\leftmarginiii\advance\labelwidth-\labelsep
    \topsep 1pt plus 0.5pt minus 0.5pt 
    \parsep \z@ \partopsep 0.5pt plus 0pt minus 0.5pt
    \itemsep \topsep}
\def\@listiv{\leftmargin\leftmarginiv
     \labelwidth\leftmarginiv\advance\labelwidth-\labelsep}
\def\@listv{\leftmargin\leftmarginv
     \labelwidth\leftmarginv\advance\labelwidth-\labelsep}
\def\@listvi{\leftmargin\leftmarginvi
     \labelwidth\leftmarginvi\advance\labelwidth-\labelsep}

\abovedisplayskip 7pt plus2pt minus5pt%
\belowdisplayskip \abovedisplayskip
\abovedisplayshortskip  0pt plus3pt%   
\belowdisplayshortskip  4pt plus3pt minus3pt%

% Less leading in most fonts (due to the narrow columns)
% The choices were between 1-pt and 1.5-pt leading
\def\@normalsize{\@setsize\normalsize{11pt}\xpt\@xpt}
\def\small{\@setsize\small{10pt}\ixpt\@ixpt}
\def\footnotesize{\@setsize\footnotesize{10pt}\ixpt\@ixpt}
\def\scriptsize{\@setsize\scriptsize{8pt}\viipt\@viipt}
\def\tiny{\@setsize\tiny{7pt}\vipt\@vipt}
\def\large{\@setsize\large{14pt}\xiipt\@xiipt}
\def\Large{\@setsize\Large{16pt}\xivpt\@xivpt}
\def\LARGE{\@setsize\LARGE{20pt}\xviipt\@xviipt}
\def\huge{\@setsize\huge{23pt}\xxpt\@xxpt}
\def\Huge{\@setsize\Huge{28pt}\xxvpt\@xxvpt}

